Theory Exploration Powered By Deductive Synthesis

Recent years have seen tremendous growth in the amount of verified software. Proofs for complex properties can now be achieved using higher-order theories and calculi. Complex properties lead to an ever-growing number of definitions and associated lemmas, which constitute an integral part of proof construction. Following this -- whether automatic or semi-automatic -- methods for computer-aided lemma discovery have emerged. In this work, we introduce a new symbolic technique for bottom-up lemma discovery, that is, the generation of a library of lemmas from a base set of inductive data types and recursive definitions. This is known as the theory exploration problem, and so far, solutions have been proposed based either on counter-example generation or the more prevalent random testing combined with first-order solvers. Our new approach, being purely deductive, eliminates the need for random testing as a filtering phase and for SMT solvers. Therefore it is amenable compositional reasoning and for the treatment of user-defined higher-order functions. Our implementation has shown to find more lemmas than prior art, while avoiding redundancy.

==> 08-future.tex <==
\section{Future Work}

\TheSy has been built from the grounds up based on term rewriting, and the results s what previous, non-symbolic tools have been able to accomplish.
However, it is our opinion that the advantages lie in its  potential to extend to new domains that cannot be
handled by concrete testing and SMT solvers.

Much of the appeal of \TheSy as a new technique for theory
exploration is its versatility in handling abstract values.
Since concrete data elements are not required for the lemma vetting process,
\TheSy can be extended to arbitrary families of types.
Our experiments have shown that it successfully handles first-class functions without generating the function bodies, but based solely on their signatures.
The next step would be to add support for refinement types~\cite{pldi91/freeman},
and notably, dependent types.
These were shown to be excellent tools in reasoning about the correctness of software~\cite{icfp14/vazou,book/cpdt,oopsla19/jad}.
In particular, their combination --- dependent refinement types --- is most interesting because it exposes the tight interconnection between types and propositions.
This makes it an ideal challenge for symbolic, constructive reasoning.

A second pain point, exposed by our experiments, is handling case splits when comparing terms as well as by carrying out proofs.
Testing technology has evolved several tools targeted specifically at handling conditional control flow in over 40 years of research in the field (\cite{cacm76/king}, with some commercial outcomes such as \cite{TaP2008:Tillman}).
The appeal of applying a proof-theoretic approach is its ability to employ mathematical abstractions to describe classes of values.
The current implementation of \TheSy essentially forks execution when splitting by case, copying the entire state.
A more careful treatment can distinguish facts that are case-specific from global ones, making the search more focused and allowing deeper proof exploration.

==> A-screening.tex <==

\section{Conjecture Inference By Symbolic Expressions}
\label{screening}

\begin{comment}
Storytelling
\begin{itemize}
    \item Difficulty
        \begin{itemize}
            \item exponential number of terms
            \item n of eq. is quadratic in number of terms
            \item checking equality is generally undecidable, and at any rate, expensive
                 (require induction)
            \item assume no base values (only ADT ctors)
                  --- cannot infer on uninterpreted / non-concrete (recursive) values
        \end{itemize}
    \item Journey
        \begin{itemize}
            \item Use PEG to compactly represent a space of terms, later we will see
              how to explore all conjectures efficiently using memoization
            \item equalities are formed not by testing all pairs, but via equivalence
              reduction; furthermore, equalities that evidently cannot be proved by
              simple induction are pruned away
            \item the equivalence relation is defined symbolically so that it can be
              computed for unknown/incomplete values
            \item inferred rules are used to further prune the space of terms by
              collapsing equivalence classes during iterative deepening.
            \item (the use of PEG helps discover common expressions during symbolic
              evaluation on example values)
        \end{itemize}
\end{itemize}


This section is all about showing 2 problems.
\begin{enumerate}
    \item There are a lot of terms and we want to save on edges
    \item There are even more equality terms and we want to filter to possible ones
\end{enumerate}

Terms as edges of terms to show subliniarity
Mention that by only checking terms and not equality terms there are quardeupaly less terms

\ldots
\end{comment}

This section deals with the first phases of the theory exploration method.
The objective is to find new conjectures using the source code without additional knowledge from the user.
Let us consider a (possibly infinite) language $\Lang$ given by a sorted vocabulary $\Vocab$.
The terms may contain free variables, with the semantics that these will be universally quantified.
For the rest of this paper, equality between terms will be definitional: two terms
$t_1, t_2 \in \Lang$ will be considered equivalent if for any valuation $\sigma$ of the 
free variables to concrete values of the appropriate types, $t_1\sigma$ and $t_2\sigma$
evaluate to the same value.

For practical reasons, SyGuS solvers usually limit generated terms by a height bound $k$.
This serves to bound the space of possible terms, and in our case, has the additional
justification that lemmas containing complex terms will be less general, and therefore,
less useful.
So the benefit of increasing the height drops for each level introduced.
The size of the space, however, grows rapidly: the size of the term space
$\mathcal{T}^{(k)} \eqdef \left\{t ~\vert~ t \in \Lang \land 
    \mathrm{height}(t) \le k\right\}$
is proportional to $\left|\Vocab\right|^k$.
This would be very large even for small vocabularies and small $k$.
Furthermore, the number of equality conjectures is quadratic in the number of terms,
roughly\footnote{this can be reduced by only considering terms of the same type, but with a relatively
small number of term types, will still be asymptotically quadratic.}
$|\mathcal{T}^{(k)}|\cdot\left(|\mathcal{T}^{(k)}-1|\right) = O{\left(|\Vocab|^{2k}\right)}$.
Checking all pairs for equality is clearly intractable.

For this reason, the goal of the screening phase is to effectively approximate the set of
valid equality lemmas and produce a small set of conjectures for the prover to check.
This must be done efficiently while maintaining a low rate of false positives, to avoid overloading
the verifier to the point where the exploration becomes infeasible.
In this section we will describe a technique to reduce the number of checked conjectures without undermining the subsequent steps of the exploration and proof process.

The main idea is to split the terms into equivalence classes whose members \emph{may} be equal for all
possible valuations, by replacing free variables with bounded symbolic values (symbolic expressions), thus over-appoximating
``real'' definitional equality.
We use a compact representation of these equivalence classes, without having to explicitly hold
all the terms in each class.
This helps mitigate the term space explosion and support efficient enumeration and symbolic evaluation
of terms for the purpose of partitioning them into classes.


\subsection{Term Evaluation Methods}
\label{screening:evaluation}

We would like an efficient term comparison procedure that is able to work without additional input from the user and is able to evaluate on all defined types, including function types.
This problem is generally undecidable, therefore solutions will always be incomplete --- meaning that
some equalities will fail to be detected --- with a tradeoff between precision and performance

The general approach taken both here and in \cite{ICAD2013:Claessen} is to enumerate through all terms, and, by evaluating them, find sets of equal terms.
From these sets, equality conjectures are derived and passed to a theorem prover for verification.

Previous work~\cite{JFP2017:Smallbone} addressed this by applying random testing with concrete values %\ES{IsaCoSy used counter example generation to do this so less relevant}.
This requires value generators for each type $\Type$ of free variables occurring in the terms being compared, and an execution environment for $\Lang$.
A generator for type $\Type$ is a function $\mathcal{F}_\Type$ generating a random distribution $\mathcal{X}_\Type$ of values from the domain of $\Type$. 
Given that all the relevant $\mathcal{G}_\Type$ are present and they created a sufficient cover of the space of input values, the correct equivalence classes will be found by using Observational Equivalence \cite{CAV2103:Albarghouthi}. %\ES{They talk about observational equivalence in quickspec. is it not enough?}.%

Although each type requires a single generator, the comparison will be limited by the distributions $\mathcal{X}_\Type$. 
The ramification is that a generic value generator may not fit every scenario, and one or more specialized generators are needed for full exploration of different vocabularies.
As an example, consider a function such as C's \texttt{strstr} that searches for an occurrence of a substring within a larger string.
The probability of generating proper substrings with plain random sampling is very low, so with
random testing, it will be hard to distinguish \texttt{strstr} from string equality.
The problem is exacerbated when free variables may take function types, such as is the case when
higher-order functions such as $\textrm{filter}$ are present in the vocabulary.

Therefore, while the random testing approach has been applied successfully before \cite{JFP2017:Smallbone,ICAD2013:Claessen,ECEASST2015:Valbuena,ITP2017:Johansson,2018AISC:Einarsdottir}, it is useful to consider a different approach. 
This work proposes to overcome these issues using a symbolic evaluation method based on term rewriting.
Using semantics-preserving rewrite rules allows to infer that terms are equal without having to
substitute concrete values for the free variables, eliminating the need for random generators.
It also allows to incorporate automatically discovered equality laws as simplification rules.
Obviously, if this inference were complete, we would not even need induction or theory exploration in
the first place.
Since rewrite-based definitional equality is inherently weak, we would not gain much by applying it
directly to the terms with the free variables.
Instead, we do substitute the variables, but with symbolic expressions that, while not representative of
\emph{all} the values of a given type, still represent \emph{infinitely many} such values.
For example, the symbolic expression $[v_1]$, with $v_1:\textrm{int}$, represents all lists of length one,
and $[v_1, v_2]$ --- all the lists of length two.

This method overcomes the limitations of using concrete values by describing (infinitely) many
concrete evaluations at once.
In fact, most if not all of the variables can be left as-is, that is, as uninterpreted values.
Only variables whose values influence the recursion depth need to be restricted.
Consider that by restricting the values relevant to recursion, the rewriting may unroll the terms until equality is found.
For example the term $map~id~[x,y,z]$ could be rewritten by the definitions of $map$ and $id$ into $[x,y,z]$.
The entire evaluation can then be carried out symbolically via a rewrite search, using known equations
$\Eqs$ as the source for rewrite rules $\RewriteSys$ and approximating $\TGroupRelationBounded{}{}{d}$
for some depth parameter $d$.
As mentioned in \autoref{overview:inference}, $\Eqs$ is initialized to the definitions of the functions
of the vocabulary $\Vocab$, but can be extended by discovered equalities, so long as these are proven
correct by \autoref{induction}, thus making the approximation tighter.

On top of that, a deductive approach can take advantage of pre-existing knowledge when analyzing new definitions.
In this way, knowledge collected by analyzing a library or a module can be used when exploring client code that interacts with that library or module.
This can enable reasoning about larger code bases without having to run all the available functions, some of which may perform expensive computations.

\begin{comment}
Also each method or value type used is defined at some time by the user, these definitions are used to create rewrite rules and later further rewrite the terms. 
There are different limitations to this type of system, first of all speed, the system needs to find matches to known rules and works as a high level interpreter. 
Another important limitation is the program space reachable with the rewrite system. 
This rewrite system proves equivalences therefor has the same limitation as provability. 
In addition to the theoretical limit there are unknown and needed rewrite rules for some comparisons, although some will be found in later iterations there is no promise all will be found. 
In order to translate even the simplest terms to equality certain rewrite rules are needed beforehand, for example \lstinline{1 + (x + 1) = (1 + x) + 1}. 
Without having a rewrite about addition being associative this equality will not be found. 
This seems like a huge limitation but as we will see later our system proves the rewrite rules it needs during its process and the function and type definitions provide most needed knowledge. 
As a result providing a set of rewrite rules for the builtins in the language is almost all user knowledge needed.
\end{comment}

\subsection{Generating Candidate Terms}
\label{generation}

In this subsection, we introduce the concept of Syntax Guided Enumeration (SyGuE).
SyGuE is similar to Syntax Guided Synthesis (SyGuS for short~\cite{DSSE2015:Alur}) in that they both use a formal definition of a language to find program terms solving a problem.
They differ in the problem definition: while SyGuS is defined as a search for a correct program over the well-formed programs in the language,
SyGuE is the problem of iterating over \emph{all distinct} programs in the language. SyGuS solvers may be improved using a smart search algorithm, while SyGuE solvers need an efficient way to eliminate duplicate terms, which may depend on the definition of program equivalence.

\begin{definition}[SyGuE]
Given a grammar $G$ and a term equivalence relation $\EquivRel$, the SyGuE problem is defined as generating all the equivalence classes of terms produced by
$G$ modulo $\EquivRel$.

\vspace{8pt}
\centering
$
    \textrm{SyGuE}(G,\EquivRel) := \big\{ \left[t_i\right] \in \Lang/\EquivRel
     ~\vert~ t_i \in \Lang_G \big\}
$
\end{definition}

Since the class $\left[t_i\right]$ may well be infinite, a representative is chosen
to stand for it.
Moreover, it is usually desirable to generate these representative terms in some
ascending order, such as by increasing size or height.
Typically, synthesizers generate terms in layers --- that is, first leaf terms
(height = 0), then iteratively create terms of height = 1, 2, etc. from the terms
of lower heights.
This technique from SyGuS is carried over to SyGuE.

\medskip

As the goal is finding equality conjectures that require induction to prove, we attempt to find all pairs of terms that might be equal.
This is done by creating all the terms and dividing them into equivalence classes using an over-approximation of the ``true'' equivalence relation, $\EquivRel$.
% should we note that finding the true equivalence relation would be great?
% lol yeah. great but hard. lets keep it lik ethis then
%We partition the space of terms
%We make sure each equivalence class contains terms that are equal for the base case of the induction; % I dont get this. I think this came too early in the paper
%look here. it doesn't make sens to write that yet
% why not?
Two terms $t_1$, $t_2$ satisfying $t_1 \EquivRel t_2$ will form a candidate for a new equation.
If we choose the relation $\EquivRel = {\TGroupRelation{}{}}\!$ (which is not an over-approximation), then $t_1$, $t_2$ are provably
equal by $\RewriteSys$.
These are the less interesting equalities: what we are really interested in
are equalities that are not directly provable using $\RewriteSys$,
but can be proven by applying induction.
%here
To this end, $\EquivRel = {\TGroupRelation{}{}}\!$ would be too strong.

Before we define the equivalence relation that we are actually going to use for this instance of SyGuE, we first describe the space of terms that will be generated.
As mentioned in \autoref{overview:inference}, at depth = 0 the synthesizer generates
a collection of placeholders $\pholder{i}{\tau~}$ for the available types $\tau$.
These placeholders will become universally quantified variables in the eventual
equations inferred, but for the time being they are treated as uninterpreted symbols
of the corresponding types.
We store them in the PEG as vertices with nullary edges (similar to $p$, $l_1$, and
$l_2$ in the example of \autoref{screening:representation}).
In addition, we create vertices for all the constants in $\Vocab$.
For each vertex, we also record its type.
These vertices constitute level 0 of the enumeration.

What follows is an iterative deepening process that is common in enumerative synthesis.
For each function symbol, $f\in\Vocab$, of type $\alpha_1\to\alpha_2\to\cdots\to\alpha_k\to\tau$
whose arity is $k$, we go over all the $k$-tuples of vertices $\langle u_1, \cdots, u_k\rangle$
such that $u_i : \alpha_i$ according to the recorded types.
We then generate a new vertex $v$ with associated type $\tau$, and the hyperedge
$\langle u_1, \cdots, u_k\rangle\xrightarrow{f}v$.
(As a common optimization, to avoid recreating terms at higher levels, we also require that
at least one of $u_1,\cdots,u_k$ be new, that is, generated at the previous level.)

\begin{comment}

To understand the creation of all terms into a compact structure, first how the terms are created is discussed, then we consider how they are merged, which is the next step in the process. To create all terms in the given language, special rewrite rules and accompanying hyper graph are created. Consider a grammar $\mathcal{G}$ of identifiers $i_j$ and accompanying types $t_j$. We separate identifiers by type, between functions and values. Starting with the hyper graph, all values in the grammar are inserted into an empty graph with their accompanying types. With the hyper graph ready we can build deeper terms using the function symbols from the grammar. Each function symbol is translated into a rewrite rule, matching parameters from the existing graph by type and resulting in a new vertex in the hyper graph, representing the created term. Practically in addition to the initial values created from the grammar, values for each type appearing in the grammar are generated, which we will refer to as placeholder values. Their purpose is to make sure all terms are created and are later on used for the equivalence step as is explained in section 2.3. For simplicity, for each type two placeholder values are created marked as $V_{p_i}$.

\begin{equation}
    \mathcal{G} := \left(\left\{v_1: t_1, v_2: t_2, \ldots, v_n: t_n\right\}, \left\{f_1: t'_1, f_2: t'_2, \ldots, f_m: t'_m\right\}\right)
\end{equation}

 

Similar to Observational Equivalence (OE), the term space is being pruned by finding equalities before creating deeper terms. Normally Observational Equivalence prunes the space by keeping only one representative from each equivalence class. In this work it is important to keep all the terms, therefor equal terms are merged in the compact structure and each vertex represents all the terms in the equivalence class. This way we gain the pruning without losing the current and future terms. Future terms refers to terms that would not have been considered in normal enumeration using OE. Let's consider the terms $x + y$ and $y + x$, they will be found equal and only one will be kept, for the example $x + y$. Future terms being created will be based on this, $1 + (x + y)$. The problem is we do not consider $1 + (y + x)$, which might make the system miss needed conjectures. Using Symbolic Observational Equivalence, both terms are kept but the new term is not yet constructed. Therefor we create only one new hyper term which will look like $1 + t \vert t \in \{x + y, y + x\}$.

There are two important points that contribute to the size of the equivalence classes in the graph. First is the merge step, which creates the equivalence classes, all the terms in a class are merged as will be explained in Section 2.3, meaning they are represented by a single vertex of the hyper graph. Later in the process the system will try to prove new lemmas, which translate to rewrite rules, these rules will be used to further merge terms. As creating the terms is done in steps, until the needed depth, the result of merging terms in the previous step will apply when creating the next level of terms. When matching the grammar rewrite rules, there are less vertexes to according to the merges that happened. Now it is not necessary to iterate all the terms created in order to produce the deeper terms, only the vertexes, which as we will see later, represent the equivalence classes.

Algorithm for term generation
\begin{enumerate}
    \item Create uninterpreted values - $val\_a_1$,$val\_a_2$, $val\_list\_a_1$, $val\_list\_a_2$ 
    \item Iterate until term depth reached
    \begin{enumerate}
        \item Iterate grammar rewrite rules
        \begin{enumerate}
            \item apply rewrite rule to hyper graph
        \end{enumerate}
        \item Use equality function to merge vertexes
    \end{enumerate}
\end{enumerate}

\ES{Choose example to run with. Show that many programs are the same like (1+1)+1 = 1+(1+1)}
\end{comment}

\subsection{Conjecture Inference}
\label{screening:soe}

%Computing equivalence classes from a given set of rewrite rules $\RewriteSys$ was described (\autoref{screening:evaluation}) $\SERelation{}{}$.

Now we describe the first part of how equivalence classes are formed and how this is used to find conjectures. Remember that our goal is to find equivalences that cannot be found in the current search space.
This cannot be done directly with the uninterpreted values $\pholder{i}{\tau}$ created above,
since most rewrite rules will have to \emph{destructure} at least one of the arguments to a function.
For example, the term $x \concat y$ has no reduxes w.r.t. the rewrites induced by the definition
of $\concat$ given in \autoref{overview:input-state}.
To overcome this, we need to introduce some structure into the values represented by the placeholders.

We generate small \emph{symbolic expressions} to be used as \emph{symbolic examples}.
They are created from the recursive data types used as placeholder types
by combining uninterpreted values from the base types and constructors.
These symbolic examples are used to discriminate programs according to their functional behavior. 
Programs that evaluate to the same (symbolic) value on all the examples are merged in the PEG. 
We take advantage of the compaction mechanism already present in the PEG data structure to detect when
symbolic values are equal, without ever having to construct those values explicitly or define a normal form.
We repeat this process for a set of possible symbolic valuations to the placeholders: for each valuation,
essentially, a working copy of the PEG is created, placeholders are filled in, and rewrites are applied up to the rewrite depth $d$.
Whenever two vertices $u_1$, $u_2$ were successfully merged in all of these derived PEGs, we merge them
in the master PEG as well to indicate that they are now considered equivalent.
This creates an ever-growing equivalence relation over the set $\Terms$ of terms generated so far.

\begin{comment}
\SI{This should go somewhere else probably}
{\color{gray}
Before explaining how the examples are generated and used, we define Rewrite Search. Rewrite Search is how we explore the term search space, by iteratively applying the known rewrite rules. After applying all the rewrite rules in iteration $i$, all proofs of depth $i$ will have been found. This means all term equalities provable with $i$ steps will be expressed as merges in the compact structure. There is no point of matching rewrite rules on the same parts of the graph twice. To prevent this we use a versioned graph and for each iteration match at least one part of the rewrite rule with the newest version of the graph.
}
\end{comment}

It would be tremendously expensive, and also unnecessary, to create all the combination of symbolic values (that would be exponential in the number of placeholders.)
Instead, we found that it is sufficient, sometimes even desirable, to only expand a single placeholder.
For the purpose of presentation, assume there is a single type $\tau$ (e.g. list) over which we plan to
perform structural induction.
We associate symbolic values with placeholder $\pholder{1}{\tau~}$, e.g.
$\pholder{1}{\tlist~T} \mapsto \left\{[], v_1\cons [], v_2\cons v_1\cons []\right\}$.
The remaining placeholders remain uninterpreted.
When multiple algebraic data types are present, the process is just repeated for each of them.

\begin{definition}[Symbolic Observational Equivalence]
\label{screening:serelation}
Given a set $\mathcal{S}_{\tau}\subseteq\Lang$ of terms representing symbolic values of type $\tau$,
We define the \emph{symbolic observational equivalence (SOE)} over terms as

\vspace{2pt}
\centering
$\SERelation{t_1}{t_2} \iff \bigwedge_{s\in\mathcal{S}_{\tau}} 
    \GroupRelationBounded{\substInTerm{t_1}{s}{\pholder{1}{\tau~}}}
                         {\substInTerm{t_2}{s}{\pholder{1}{\tau~}}}{d}$
\end{definition}

That is, then the symbolic values of $t_1$ and $t_2$ converge for all the symbolic values $\mathcal{S}_{\tau}$ that $\pholder{1}{\tau~}$ can take.
Equality between symbolic values is determined by a rewrite search of depth $d$.

\begin{paragraph}{Automatic case-splitting.~~}
Even with a single induction variable, and with size-bounded symbolic values,
symbolic evaluation can get blocked and cripple the equality checks.
This is a known phenomenon stemming from the presence of conditional branches
in definitions.
For example, in the expression $\tfilter~p~(v_1\cons {[]})$, the definition
of $\tfilter$ would introduce a term of the form
``$\tmatch~(p\,v_1)~\twith~\cdots$''.
Evaluation cannot continue without knowing the value of $p\,v_1$.
The rewrite-based comparator overcomes this using a split-case, in a way
that is commonly employed by symbolic execution environments~\cite{OSDI2008:Cadar,CACM2013:Cadar}
Evaluation is \emph{forked} and both branches explored, where each fork
assumes an additional \emph{path condition}:
\textit{e.g.}, one fork assumes $p\,v_1=\tfalse$, and the other
$p\,v_1=\tfalse$. Two terms will then be merged only if they are merged
on both forks.

Evidently, the number of forked states grows exponentially with the number
of conditions that may be encountered during evaluation.
It is important to apply split-case judiciously, so a tighter bound is 
placed on the number of nested forking steps than the bound $d$ on
regular rewrite steps.
Luckily, a small number of split is sufficient in many scenarios.
Consider the following two terms from the running example in \autoref{overview:inference} \eqref{overview:example-terms}.
\[
\tfilter~\pholder{1}{T\to\tbool}~
(\pholder{1}{\tlist\,T} \concat \pholder{2}{\tlist\,T})
\qquad
(\tfilter~\pholder{1}{T\to\tbool}~\pholder{1}{\tlist\,T})
~\concat ~
(\tfilter~\pholder{1}{T\to\tbool}~\pholder{2}{\tlist\,T})
\]

So the screener will have to compare, \textit{e.g.},
\[
\tfilter~p~\big((v_1\cons{[]}) \concat l_2\big) ~~\maybeEq~~
{\big(\tfilter~p~(v_1\cons{[]})\big)} \concat {(\tfilter~p~l_2)}
\]

While $\tfilter$ would eventually apply $p$ to all the elements of
both $v_1\cons{[]}$ and $l_2$, it is enough to split into two cases:
when $p\,v_1=\ttrue$, both terms evaluate to
$v_1 \cons {\tfilter~p~l_2}$; when $p\,v_1=\tfalse$, they both evaluate to
$\tfilter~p~l_2$.

\end{paragraph}

\medskip
% This concludes this section
At the end of each iteration, every vertex represents an equivalence class defined by the rewrite search modulo the set of symbolic valuations that was used.
At this point we can say that all combination of two terms from a single class can be an equality conjecture, which still has to be checked by the prover since the symbolic examples still do not cover \emph{all} possible inputs.
This leads to the next part of the process where we further filter the conjectures and try to prove the ones left using induction.


==> B-induction.tex <==
\section{Induction by Deduction}
\label{induction}

This section describes the final conjecture filtering and proof attempt process.
After running Symbolic Observational Equivalence (\autoref{screening:soe}), equivalence classes created from symbolic examples are obtained.
Terms that were found equal by the approximation (using rewriting) of $\SERelation{}{}$ might be provably equal without requiring induction.
At this point it is needed to create finer classes by a relation unifying conjectures that are provable without induction.

Our experiments show that this filtering passes through a small set of candidate lemmas.
We use the same rewrite search to discharge the induction step.
While simple, we found it to be quite robust when integrated with the exploration system as a whole.
Instead of guessing auxiliary lemmas that are needed to carry a proof to
completion, we rely on discovery of provable lemmas during search.
The robustness also stems from an ordering of the conjectures being explored.

\subsection{Refining Equivalence Relation}

Given a set of terms $\Terms$, we start by building an over approximation of the provable term equalities. 
This is done by approximating the equivalence class $C \in \Terms / \SERelation{}{}$ (see \autoref{screening:serelation}).
As mentioned, this step is meant to screen out conjectures that do not require induction to prove, before applying induction, which can be done given the current set of rewrite rules $\RewriteSys$.
This screening helps in preventing addition of unneeded rewrite rules into $\RewriteSys$, keeping it minimal and reducing run time.

We screen the conjectures by taking all the terms in $C$ and create a finer partitioning $C_F = C / \underset{C}{\xleftrightarrow[]{\RewriteSys}}^{\!(d)}$.
Note that as the equivalence classes are represented in the compact structure (\autoref{screening:representation}), they are all represented by a single vertex.
Therefore, to be able to perform rewrite search and find the finer classes, it is needed to reconstruct the terms into a new compact representation, where each term is represented by a different vertex.
We still wish to reduce the amount of terms we enumerate; although it does not affect the asymptotic complexity of the problem, it results in significant speedups.
The reconstruction is done bottom-up, taking advantage of memoization for common subterms (which are numerous), reducing the amount of edges that have to be inserted to the graph.

\newcommand\tgood{\textit{good}}
\newcommand\tbad{\textit{bad}}

By creating $C_F$ using a rewrite search, we take advantage of the fact that running a rewrite search and finding that $t_1 = t_2$ constitutes as a proof.
This is true when uninterpreted values are used, as is the case in while approximating $C_F$.
From the definition of $C_F$ all terms in $\left[ t_j \right] \in C_F$ are proven to be equal to each other by the rewrite search.
For each such $\left[ t_j \right]$ we want to choose a single representative.
This representative term will be used in creating final conjectures to be passed to the prover.
It actually matters which representative we choose, although they were proven equal.
Consider the conjecture $c_{\tgood} := x + y = y + x$, we could have chosen different representatives and write it as $c_{\tbad} := 0 + x + y = 0 + y + x$.
The chosen representative will affect the created rewrite rule.
Choosing the larger term might lead to a rewrite rule that won't match all needed contexts while applied.

At this phase our main concern is to choose the representatives and order the conjectures well. 
We want to avoid having both rules $c_{\tgood}, c_{\tbad}$ are proven, or worse, having $c_{\tbad}$ proven and $c_{\tgood}$ discarded because it is redundant.
Continuing with the example, if $c_{\tbad}$ was proved before $c_{\tgood}$, it means $c_{\tbad}$ is now represented in $\RewriteSys$.
During a screening, $c_{\tgood}$ will be deemed unnecessary due to the presence of $c_{\tbad}$.
This can happen since the following is a valid rewrite chain:
\[x + y \xrightarrow{x = 0 + x} 0 + x + y \xrightarrow{c_{\tbad}} 0 + y + x \xrightarrow{y = 0 + y} y + x\] 

Because the system has a feedback loop, during which the lemmas proved are used again for later proofs, it is important to avoid such bad choices.

We define ordering on terms in an effort to always choose first the term that will match the most situations. 
We define order over the terms first by size (smallest first), then by generality (most variables first).
\begin{definition}[Term Ordering]
\label{induction:ordering}
For a term $t\in\Lang$, let $|t|$ denote its size, that is, the number of
AST nodes in its syntactic representation.
We define a preference ordering $\preceq$ of terms lexicographically over
the tuple $\big\langle|t|, |\FV(t)|\big\rangle$, where term sizes are compared with $\leq$
and free variable sets sizes are compared with $\geq$.
\[t_1 \preceq t_2 \iff \big\langle|t_1|, |\FV(t_1)|\big\rangle
    \underset{\scriptscriptstyle (\leq,\geq)}{\leq}
    \big\langle|t_2|, |\FV(t_2)|\big\rangle\]
\end{definition}
We then use this ordering as a heuristic to choose a representative from each $\left[ t_j \right] \in C_F$, which will be minimal according this order.

The overall process can be described as running a $SyGuE(G, \SERelation{}{})$
followed by $SyGuE(G_{[t_j]}, \GroupRelationBounded{}{}{d})$
for each of the equivalence classes, where $G_{[t_j]}$ is the input grammar restricted to the equivalence class $[t_j]$.
Finally, enumerating the resulting representatives is much less than all the pairs in each $[t_j]$
and definitely much less than $|\Terms|^2$.

\subsection{Induction Step}

The last step of each iteration in this process is attempting to prove the conjecture using induction.
Given the equivalence class $C$ and representatives for each fine equivalence class $\left[ t_j \right] \in C_F$, a conjecture is built as $c := t_1 = t_2$ for each combination two representatives.
As will be shown in the results, only a small amount $\left[ t_j \right]$ classes exist foreach $C_F$, which goes to show this screening technique is effective. 
For each conjecture $c$ we already know at this point that $t_1$ is \emph{not} provably equal to $t_2$ in $d$ rewrite steps.
This is the point in the process that we assume that an induction proof is needed. Each conjecture is used as the induction hypothesis of the proof;
intuitively, if there is a need for a stronger induction hypothesis,
we rely on the system itself to eventually discover a sufficient auxiliary lemma.
\begin{comment}
at the past or at the future the system will prove it as a lemma and that knowledge will become available for the induction step.
Still, some lemmas only will obviously be impossible to find with this limitation, for example using a precondition $x > y$, $max(x,y) \quad \overrightarrow{x > y} \quad x$. Currently such a condition will need to arise from how functions are defined by in the given input. 
\end{comment}

At this point only the induction step is needed.
The reason for that is that base cases for the induction proof were already taken care of in \autoref{screening:soe}. 
This happens when the examples are proved to be equal, which include all the base cases of the inductive data type. It remains to carry out the induction step.

Given the conjecture $c := t_1 = t_2$, during induction on type $\Type$, there is a need for induction step proof for each constructor $\ctor_k(v_1, \ldots, v_{n_k})$ of $\Type$.
We construct a search space representing the proof obligation for $\ctor_k$, to be dismissed using rewrite search.
The search space is just the compact structure containing the terms $t_1, t_2$ \footnote{Recall that some of the rewrite rules are directed, requiring that both terms be included.}, which are updated to represent a step using $\ctor_k$.
The induction variable will always be chosen as the first placeholder value for the type $\Type$ which we will refer to as the induction variable or $iv$.
A term $t$ will be updated by substituting $t[\ctor_k(v_1, \ldots, v_{n_k})/iv]$ where the constructor parameters are new uninterpreted variables of the appropriate types.
We define a well founded order $\ltwf$, to automatically recognise terms that are sub-structures of $iv$ to
which the induction hypothesis can be applied soundly.
For example, given $iv = v_1 \cons v_2$ (for $v_1 : \Type$, $v_2 : \tlist\,\Type$), we have $v_2 \ltwf iv$.
Both the hypothesis and the order $\ltwf$ are represented as rewrite rules added into $\RewriteSys$.
Some proofs will require that the inducted value will be in a certain position in the term, \textit{e.g.} the first or the second argument
to a recursive function. 
This is solved ahead of time by generating all possible terms, as we also generate a term with the placeholder in the right position for the induction.

%Even if the proof will succeed sometimes it is not enough.
The order of the conjectures being tested can affect the results of the theorem search.
Consider plus associativity, the system can find that $c_1 := x + (y + z) = (x + y) + z$ and also that $c_2 := x + (y + x) = (x + y) + x$.
If we succeed in proving $c_2$ before $c_1$, we will end up with an unneeded lemma.
However, by proving $c_1$ first and adding it to $\RewriteSys$, we can dismiss $c_2$ as it can be obtained from $c_1$ without induction.
The first step to solving this is using the order defined in \autoref{induction:ordering}.
Another problem that may arise is proofs failing due to insufficient rewrite rules.
Take the example of $\tfold$ and $\tsum$ (\autoref{induction:foldsum}).
The following three conjectures are at play:
%
\begin{align}
\label{induction:conjfoldsum}    
 c_1 &~:= & \tfold ~ (+) ~ 0 ~ l &= \tsum ~ l     & & \\
 c_2 &~:= & x + \tfold ~ (+) ~ 0 ~ l &= \tfold ~ (+) ~ x ~ l  & & \nonumber \\
 c_3 &~:= & x + \tfold ~ (+) ~ 0 ~ l &= x + sum ~ l   & & \nonumber
\end{align}

Before proving the conjecture $c_1$, the conjecture $c_2$ needs be proved.
Due to the ordering, first the smaller conjecture's proof, i.e. $c_1$ will be attempted and will fail, then $c_2$ will be proved.
Without any further rearrangement of the conjectures, a proof attempt of conjecture $c_3$ will succeed. 
This makes the system find that $c_1$ is unnecessary and will prevent the system from proving it.
\begin{comment}
\ES{We've already been through such an explanation so seems redundant to put this here}
This happens because during the screening phase both
$\tfold ~ (+) ~ 0 ~ \pholder{1}{\tlist\,\tnat}$ and 
$0 + \big(\tfold ~ (+) ~ 0 ~ {\pholder{1}{\tlist\,\tnat}}\big)$ 
are in the same fine equivalence class.
\end{comment}

Order is very important in this system, therefor if a lemma is found, all conjecture proofs that were failed to this point are reattempted.
Before reattempting proof for a conjecture $c$, we recheck if the conjecture $c$ is still needed by running a rewrite search over the terms of $c$.
This way the system returns to the original smaller conjecture and succeeds in proving it finding \iterm{$\tfold~(+)~0~l = \tsum~l$}, making 
$c_3$ redundant, thus proving only the smallest needed theorems for this case.

This proof technique is robust as it can work for user defined functions and data structures, while proving the needed auxiliary lemmas on the run. 
Although most of the proof process is dependant on the previous steps, the induction proof is independent of it's predecessors. 
This means that any proof technique that can work with two given terms can be used instead. 
Having said that the naive approach solved all the needed proofs and does not majorly affect the run time. 
As only a few term combinations reach this stage the run time of a single proof search is of little affect on the total system run time.

\begin{example}{Proof of \eqref{induction:conjfoldsum}$c_1$ --- $\tfold ~ (+) ~ 0 ~ l = \tsum ~ l$ by induction on $l$, once \eqref{induction:conjfoldsum}$c_2$ has been proven.}
\label{induction:foldsum}
\vspace{-3mm}
\[
\renewcommand{\arraystretch}{1.3}
\newcommand\xs{\mathit{xs}}
\begin{array}{l@{\quad}l}
\textit{Assume} & 
\tfold~(+)~0~\xs = \tsum~\xs
 \\[.5em]
\textit{Induction Step}
    & \tfold ~ (+) ~ 0 ~ (x\cons\xs) \Rightarrow \tfold ~ (+) ~ (0 + x) ~ \xs 
      \Rightarrow \tfold ~ (+) ~ x ~ \xs \\
    & ~~\overset{c_2\,}{\Longrightarrow}  x + \tfold ~ (+) ~ 0 ~ \xs \overset{\textrm{IH}\,}{\Longrightarrow}
    x + \tsum ~ \xs \Rightarrow \tsum~(x\cons \xs) \\[-.75em]
\square &
\end{array}
\]

Notice that this example, variants of which occur in some tutorials on
formal proofs using proof assistants, typically requires a strengthening
of the inductive property.
This was completely avoided here thanks to the auxiliary lemma, which was automatically discovered.
\end{example}

\begin{comment}
\begin{example}{Proof of $\reverse(l \snoc x) = x :: \reverse(l)$ (Equation \eqref{induction:conjfoldsum}) by
induction on $l$.}
\renewcommand{\arraystretch}{1.2}
\[
\begin{array}{lll}
    \textnormal{Base Step:} &l& = nil \\
    && \reverse(nil \snoc x) \Rightarrow \reverse(x :: nil) \Rightarrow 
       nil \snoc x \\
    &&\Rightarrow  x :: nil \Rightarrow x :: \reverse(nil) \\[.5em]
    \textnormal{Induction Step:} &l& = y::l_1 \\
    && \reverse(y :: l_1 \snoc x) \Rightarrow \reverse(l_1 :+ x) \snoc y \\
    && \Rightarrow x :: \reverse(l_1) \snoc y \Rightarrow x :: \reverse(y :: l_1)
\\
\end{array}
\]
Note: The rewrites used are only from the definitions of the functions ($\snoc$ and $\reverse$).
\end{example}
\end{comment}

==> Z-results.old.tex <==
\section{Evaluation}
\label{results}

Evaluating a theory exploration system poses some challenges.
One challenge is that different combinations of lemmas can be used to express the same knowledge (in the sense that was described in \autoref{overview}).
Testing whether a discovered theory expresses the correct and full knowledge expected could be done by checking that the knowledge obtained from exploration subsumes the expected knowledge. 
However, this check is not feasible because, essentially, $\mathcal{K}_\mathcal{T}^S$ is infinite; notice that it is not sufficient to check whether all of the lemmas in some $\mathcal{T}_1$ can be proven using some other $\mathcal{T}_2$. There may still be some formula $\varphi$ such that $\mathcal{T}_1 \vdash^S \varphi$ but  $\mathcal{T}_2 \not\vdash^S \varphi$ --- due to bounds necessarily imposed on proof search in order to guarantee termination.
For this reason, we resort to a manual investigation of the result relative to a set of known lemmas that we expect to be found (for example, $l_1\concat {[]} = l_1$).
Another challenge arises when comparing with existing tools for automated reasoning since different tools work in different scenarios in which they expect different kinds of user input.
As a principal, our design goals for \TheSy was to perform exploration using function definitions alone without additional user guidance.
This affects the interpretation of any comparison to theorem provers or verification systems such as Leon, as the input is meaningfully different.
To evaluate \TheSy we compare with Hipster~\cite{CICM2014:Johansson}, a fully automated exploration system with several follow-ups \cite{ECEASST2015:Valbuena,ITP2017:Johansson,2018AISC:Einarsdottir}.

As a comparison of \TheSy and Hipster requires manual analysis, we perform a case study of a handful of test cases that we consider representative, while adding a discussion of the results for each of them and how they relate.
Besides that, all lemmas found during exploration are inserted to Leon to attempt to verify them.
This last step is also a demonstration of how theory exploration can strengthen and augment software verification.

We present the implementation details and experimental setup, then move to showcase the capabilities of \TheSy using a collection of benchmarks that is representative of functional programming practices. These are shown independently of preexisting tools.
This is followed by a discussion of the comparison with other systems.

\subsection{Implementation and Setup}
\label{results:implementation}

As \TheSy relies heavily on term rewriting, there are a few additions to our implementation of the PEG data structure to improve performance.
The rewriting engine is incremental, relying on the PEG supporting incremental processing:
Our incremental PEG keeps track of when edges are added, and during the pattern match step of rewrite rule application, at least one matched edge should be new; that is, it has been created after the last time that rule was applied.
This optimization avoids recomputation of pattern matching across the ever-growing hypergraph, and prevents unnecessary edge insertions and node merges.

\begin{comment}
When running SOE, all the different symbolic valuations are inserted into the hypergraph at once, 
and the hypergraph is duplicated for each valuation to keep terms on different valuations distinct.
By combining the duplicated hypergraphs into one, there is sharing of the symbolic term evaluation for all valuations.
We reuse uninterpreted values when creating larger symbolic expressions (actually, the whole example is reused). 
By which taking advantage of the term sharing to reduce the amount of rewriting needed.

For example consider the valuations for list $[], [x], [y,x]$, both $[]$ and $[x]$ are reused.
As a result, when evaluating a term, for example $rev$, less steps are needed as it reuses the calculations for the smaller valuation.
\[ rev([]) \rwto [] \quad rev([x]) \rwto rev([]) :+ x \quad rev([y,x]) \rwto rev([x]) :+ y \]
\end{comment}

\begin{comment}
\TheSy also applies different rewrite rules in parallel, providing some additional speedup.
This speedup is vital when the knowledge base grows, meaning more lemmas exist, as each lemma gets translated into a rewrite rule.
By matching and concluding in parallel, rules that are irrelevant to the current context fail to match instantly and do not slow down execution.
The compaction operation, however, is sequential, and it currently dominates the running time.
There is definitely room for further implementation improvements to accelerate the performance-critical parts.
\end{comment}

As mentioned, \TheSy supports automatic case splitting; this is done for functions that contain $\tmatch$ expressions ($\tif$ is just a special case of $\tmatch$). 
A special rewrite rule is created to enable split cases during term evaluation, by marking terms to split and split values. 
For each split marker and relating split values, it copies the hypergraph for each split value, replacing the marked term with the split value. 
Case splitting is done recursively, performing rewrite search on each split value for each level until reaching the maximum split depth. 
After finishing the search for all branches, conclusions are merged to find what equalities were proved.
This implementation results in repeating the same branches due to the ordering, which worsens with deeper split depth. 
As there is no consideration of whether a case split will be useful, depending on where it is applied, many unnecessary case splitting is done.
While limiting scale in its current format, \TheSy was able to find lemmas about the functional operator `$\tfilter$' with small vocabularies.

\TheSy has a few control parameters governing the term generation and search processes.
For experiments in which we use non-default parameters, the decision is explained in the following discussion.
Now we review the parameters and their impact on the exploration results.
The rewrite search depth $d$ affects what equalities we might find: A shallow search can lead to missed lemmas,
but deeper search may be prohibitively expensive as some of the rewrite rules can run infinitely, such as in the case of $x \rightarrow x + 0$.
The default search depth is $d = 8$. 
Terms are always generated up to depth 2 ($k = 2$).
The symbolic expressions used for discriminating terms are created with a maximal depth of 2 ($c = 2$).
When using the case split feature, larger symbolic expressions will require increasing the maximum split depth, therefore in those cases, $c$ is reduced to 1.
(This reduction negatively impacts the robustness of the inference phase; \eg, $\treverse~l_1=l_1$ for lists of size 1. These spurious lemmas will have to be discarded by the induction prover.)

All benchmarks were executed on a Xeon E3-1231 v3 (quad-core) machine with 32GB of RAM.

\subsection{Experimental Results}
\label{results:experimental}

The cases being checked are defined by the sorted vocabulary used, which encapsulates the relevant functions and data type definitions.
For each experiment, we report the number of lemmas which were: found and proven, passed screening but failed the proof, and those for which proof succeeded only on retry.
If a proof failed when a lemma was first discovered, but succeeded later on, it means that a necessary auxiliary lemma was found and that lemma enabled the proof to go through.
This situation is common as auxiliary lemmas are sometimes larger and occur later in our ordering.

Some of the lemmas proven in early test cases are reused later to prevent \TheSy from reproving lemmas. 
Lemmas for $\lor$ and $\land$, which do not require induction to prove, are also encoded as rewrite rules.
(\TheSy can in fact prove them, but they are discarded during screening for being to simple.)

The experimental results are listed in \autoref{eval:all-lemmas}, where for each given vocabulary all the lemmas found by TheSy are presented. Additionally a breakdown of the run time is presented in \autoref{table:experiments}. As the term generation and conjecture inference phases are highly coupled and as the term generation is relatively insignificant, the total time for both phases is presented.
The conjecture screening phase happens many times, as it is needed when proofs are retried.
We therefore seperate its run time from the prover, presenting the accumulated time spent screening.
The prover column includes two measurements. 
The left one is the total time spent on in the prover.
The left represent the amount of time, from the total time in the prover, spent on retrying to prove a conjecture.
All the measurements are given in seconds.

There are two measurements given for experiments containing $\tfold$ in the vocabulary.
When using the default parameters, \TheSy creates many unneeded terms for those cases.
To demonstrate the impact of this, we added a second run, reducing the number of placeholder values created.
Certainly, it is possible to optimize all experiments by choosing the correct parameters, but the goal remains to work fully automatically therefor it is preferred to keep the defaults.

Another design choice impacting performance is adding a conjecture filtering phase, in the end of the iterative deepening, after finding new rules.
This is important as was shown in the end of the overview (\autoref{overview}), as it allows finding new lemmas.
The additional knowledge, discovered during the exploration, helps the conjecture inference phase discover more equalities.
The effect on run-time can be astronomical when working with larger vocabularies.
This is because continued rewriting of large hypergraphs becomes resource expensive as they keep growing.
For example, considering the stress test, finding the lemma -- $\tmap~f~(\trev~l) = \trev~(\tmap~f~l)$ -- is possible due to this additional run, which changed the run-time from ~1 hour to ~4.
Still, when considering theory exploration, the additional lemma can be very useful for the future and should not be overlooked.

A few concepts are displayed in the experimentation.
\begin{itemize}
    \item Being able to find basic facts about new data types such as Nat, List, and Tree.
    \item The ability to explore higher-kind functions such as filter map and fold.
    \item Working with bigger vocabularies as seen in the stress test
    \item Knowledge transfer, some of the experiments successfully reuse knowledge to find new results (this can be seen in the "filter ++" test that uses facts on ++).
\end{itemize}

\begin{table}
\resizebox{\textwidth}{!}{
\input{tables/all-lemmas}
}
\caption{A list of the lemmas that were discovered using different vocabularies ($\Vocab$).}
\label{eval:all-lemmas}
\end{table}

\begin{table}[t]
\resizebox{0.9\textwidth}{!}{
\input{tables/experiment-stats}
}

\smallskip
\caption{Statistics for evaluation benchmarks.
In each experiment, we report the total number of lemmas found, as well as candidates that passed the initial screening but failed the prover, and the number of proof retry attempts.
Numbers in parentheses represent faster runs with tweaked parameters (see text).
}
\label{table:experiments}
\end{table}

\subsection{Comparison}
\label{results:comparison}

To compare the performance of \TheSy to that of existing tools, we selected a set of sorted vocabularies that we believe express different aspects and difficulties in theory exploration.
These include different ADTs (lists trees and naturals), lemmas that rely on auxiliary lemmas for their proofs, and conditional lemmas (the latter are currently not supported by \TheSy but are nevertheless a pervasive component in automated theorem proving.)
We compared \TheSy with Hipster~\cite{ITP2017:Johansson}, a theory exploration add-on for Isabelle/HOL, and Leon~\cite{SCALA13:Blanc}, a verification and synthesis tool for Scala.
All three share a domain of purely functional programs with algebraic data types and recursive definitions.
We added Leon to our comparison to see which of the lemmas can be automatically proved without further intervention;
meaning whether exploration can be beneficial and prove or help prove lemmas that are not trivial for it.
As the theory exploration systems stop when they finish exploring defined space, we added a timeout of half an hour for Leon to keep the comparison close.
\autoref{eval:case-study} shows the results of running the three tools on different vocabularies.

Following is a case study comparing the three systems. 
Some cases benefit from using previously obtained knowledge, so results from previous cases are retained.
During the study, Hipster and \TheSy receive only the sorted vocabulary, while in Leon we also add the lemma definitions as it has no concept of theory exploration.
As we can see in the results, there are many cases, usually the more intricate ones, in which the exploration can serve a system like Leon.

\begin{table}
\centering
\resizebox{0.98\textwidth}{!}{%
\input{tables/case-study}
}

\vspace{2pt}
\caption{Results of the case study comparing \TheSy, Hipster, and Leon}
\label{eval:case-study}
\end{table}

\begin{myparagraph}{Case study 1 --- natural numbers.}
We included the canonical construction of natural numbers based on $0$ and $\tsucc$ (successor) and a recursive definition of $+$.
By default, two placeholders are created per type. $+$ has two arguments of the inducted type, requiring three placeholders to fully explore the space.
If only two placeholders were used, commutativity ($x+y=y+x$) can be discovered, but not associativity ($x + (y + z) = (x + y) + z$). With two placeholders, \TheSy can find only limited cases such as $x + (x + y) = (x + x) + y$.
Therefore, the number of placeholders used for this vocabulary is increased to $3$.
\TheSy and Hipster found the same knowledge, with a slight difference.
\TheSy added an extra, unneeded lemma for $x+1$.
It happened due to the ordering of the lemmas, where the smaller is added first.
Leon cannot prove commutativity as it requires an auxiliary lemma; although Leon proved the lemma, it requires user intervention to use it.
\end{myparagraph}

\begin{myparagraph}{Case study 2 - lists.}
This experiment involves polymorphic lists constructed with $[]$ and $\cons$, and the definitions of $\concat$ (list concatenation) and $\trev$ (reverse).
As $\concat$ is present in the vocabulary, with a signature containing the inducted type in more then one argument, similar to Case 1 but here more function symbols are present. 
In this case \TheSy runs twice, building basic knowledge on $\concat$ alone with 3 placeholders and only later runs on the full vocabulary with the default parameters.
In this setting, \TheSy discovers commutativity and associativity of $\concat$, as well as a distributivity with $\trev$ ($\trev~(l_1 \concat l_2) = \trev~l_1 \concat \trev~l_2$) and the nice property $\trev~(\trev~l_1) = l_1$.
Hipster generates most of the expected results but fails to discover $\trev~(\trev~l_1) = l_1$.
Hipster did find a similar lemma, $\trev~(l_1 \concat \trev~l_2) = l_2 ++ \trev~l_1$, which when instantiated with $l_1=[]$, implies the expected lemma. However, requiring this extra reasoning step makes the lemma harder to use in automated provers as well as in interactive environments.
We do note that when we re-ran Hipster with $\Vocab=\{\trev\}$, then, based on lemmas discovered in the previous step, Hipster recovers the missing lemma.
The additional execution leads to a total runtime of 18 minutes.
Leon manages to verify the simple auxiliary lemmas while failing at those that require using them.
\end{myparagraph}

\begin{myparagraph}{Case study 3 --- functional operators.}
With the basic functional primitives for lists $\tmap$ and $\tfilter$, along with $\concat$ from before, \TheSy successfully discovers distributivity properties. Hipster fails to discover these properties.
Hipster can find the comutativity lemma $\tfilter~p~(\tfilter~q~l_1) = \tfilter~q~(\tfilter~p~l_1)$, which \TheSy was unable to reach due to the number of case splits required by $\tfilter$ (as a consequence of the conditional statement in the definition of $\tfilter$).
With $\tfilter$ alone, \TheSy can recover this property in ~7 seconds via an additional case-split depth.
With $\tmap$ and $\concat$ alone, \TheSy finds the same lemmas in ~40 seconds.
This case study shows the importance of automatic case splitting when reasoning about functional programs.
Further research and engineering effort should lead to more efficient treatment of this aspect, enabling a full exploration of theories containing $\tfilter$ and similar functions.
The lemmas found in this case study can be proven without any support lemmas, and Leon succeeded in proving all of them.

We then explored a third functional operator, $\tfold$.
(As an aside, libraries often contain efficient implementations of $\tfold$, so rewriting a user program using $\tfold$ can significantly improve its performance; this was one of the motivations for this case study.)
\TheSy finds four lemmas, one of which is, in fact, redundant (due to an implementation bug).
Hipster finds a single lemma, showing the equality of $\tfold~0~+$ and $\tsum$ but again, includes redundant symbols ($x + (\tsum~y)$ instead of $\tsum~y$).
$\tfold$ is another case where having many placeholders is unfavorable to \TheSy's run time.
If we limit the number of placeholders to one per type, TheSy finishes in 42 seconds.
Leon is unable to prove any lemma in this case.
\end{myparagraph}

\begin{myparagraph}{Case study 4 --- trees.}
An important aspect is dealing with custom data structures.
This case investigates the behaviour over an additional data structure to check the effect on run time. 
All tools succeed in this, although it does not contribute much to the comparison it does demonstrate to the reader the robustness of the exploration.
\end{myparagraph}

\begin{myparagraph}{Case study 5 --- conditions.}
A difficult challenge in theory exploration is creating conjectures containing logical implications, as this quickly leads to space explosion.
By allowing the user to provide predicates to use as premises, it is possible to reduce the lemma space significantly, while retaining suitable conjectures.
\TheSy does not yet support this feature, and therefore, cannot produce such lemmas.
Hipster uses a feature from QuickSpec to generate conjecture based on given predicate \cite{ECEASST2015:Valbuena}.
This works well in the context of $leq$, but is limited for other forms of predicates (such as \texttt{strstr} as described in \autoref{screening:evaluation}).
\end{myparagraph}


==> tables/all-lemmas.tex <==
\renewcommand\arraystretch{1.1}
\begin{comment}
\begin{tabular}{@{\hspace{3mm}}l|ll}
$\Vocab$ & \multicolumn{2}{c}{Lemmas discovered} \\
\hline
$\trev ~ \cons ~ \snoc$
  & $x \cons \trev~l_1 = \trev~(l_1 \snoc x)$
  & $\trev~(\trev~l_1) = \trev~l_1$ \\
\hline
$\cons ~ \concat$ &
    $ (l_1 \concat l_2) \concat l_3 = l_1 \concat (l_2 \concat l_3) $ \\
\hline    
$\cons ~ \concat ~ []$ &
    $ l_1 \concat [] = l_1 $ \\
\hline
$\tfilter$ &
    $ \tfilter~p~(\tfilter~p~l_1) = \tfilter~p~l_1 $
  & $ \tfilter~p~(\tfilter~q~l_1) = \tfilter~q~(\tfilter~p~l_1) $ \\
\hline
$\trev ~ \cons ~ \snoc ~ \concat$ 
  & $ \trev~(\trev~l_1) = l_1 $ \\
  & $ \trev~(l_1 \snoc x) = x :: \trev~l_1 $
  & $ \trev~(l_1 \concat l_2) = (\trev~l_2) \concat (\trev~l_1) $ \\
\hline
$0 ~ \tsucc ~ +$
  & $ x + 0 = x $
  & $ \tsucc~x = x + (\tsucc~0) $ \\
  & $ \tsucc~x + y = x + \tsucc~y $
  & $ (x + y) + z = x + (y + z) $ \\
  & $ x + y = y + x $ \\
\hline
$\tfilter ~ \concat$
  & $ \tfilter~p~(\tfilter~p~l_1) = \tfilter~p~l_1 $ 
%  & $ \tfilter~p~(\tfilter~q~l_1) = \tfilter~q~(\tfilter~p~l_1) $ 
  & $\tfilter~p~(l_1 \concat l_2) = \tfilter~p~l_1 \concat \tfilter~p~l_2 $ \\
\hline
$0 ~ + ~ \tfold ~ \tsum$
  & $ \tfold~(+)~0~l_1 = \tsum~l_1 $
  & $ \tfold~(+)~x~l_1 = x + \tsum~l_1 $ \\
   % $ \tfold~(+)~x~l_1 = x + \tfold~(+)~0~l_1 $ \\
   % $ x + \tsum~l_1 = x + \tfold~(+)~0~l_1 $
\hline
$\ttrue ~ \tforall$
  & $ \tforall~l_1 = \tfold~(\land)~\ttrue~l_1 $
  & $ \tforall~l_1 \land b = b \land \tfold~(\land)~\ttrue~l_1 $ \\
$\land ~ \tfold$
  & $ \tforall~l_1 \land b = \tfold~(\land)~b~l_1 $
  & $ b \land \tfold~(\land)~\ttrue~l_1 = \tfold~(\land)~b~l_1 $ \\
\hline
$\tfalse ~ \texists$
  & $ \tfold~(\lor)~\tfalse~l_1 = \texists~l_1 $
  & $ \tfold~(\lor)~b~l_1 = b \lor \tfold~(\lor)~\tfalse~l_1 $ \\
$\lor ~ \tfold$
  & $ \tfold~(\lor)~b~l_1 = \texists~l_1 \lor b $
  & $ b \lor \tfold~(\lor)~\tfalse~l_1 = \texists l_1 \lor b $ \\
\hline
$\tmap ~ \circ$
  & $ \tmap~f~(\tmap~g~l_1) = \tmap~(f\circ g)~l_1$ \\
\hline
$0 ~ 1 ~ + ~ \trev ~ \snoc ~ \tlen$
  & $ \tlen~(l_1 \snoc 1) = \tlen~(l_1 \snoc 0) $
  & $ 1 + \tlen~l_1 = \tlen~(l_1\snoc x)$ \\
  & $ \tlen~(\trev~l_1) = \tlen~l_1$
  & $ \tlen~(l_1\snoc x) = \tlen~(l_1\snoc 0)$ \\
  & $ \tlen~(l_1\snoc x) = \tlen~(l_1\snoc 1)$
  & $ 1 + \tlen~l_1 = \tlen~(l_1\snoc y)$ \\
\hline
$+ ~ \concat ~ \tlen$
  & $ \tlen~(l_1 \concat l_2) = \tlen~l_1 + \tlen~l_2 $ \\
\hline
$\tmap ~ \cons ~ \snoc ~ \trev$
  & $ \tmap~f~(l_1 \concat l_2) = \tmap~f~l_1 \concat \tmap~f~l_2 $
  & $ \trev~(\trev~l_1) = l_1 $ \\
$\concat ~ \tfold$
  & $ \trev~(l_1 \concat l_2) = \trev~l_2 \concat \trev~l_1 $
  & $ \tfold~f~(\tfold~f~x~l_1)~l_2 = \tfold~f~x~(l_1\concat l_2) $ \\
  & $ x \cons \trev~l_1 = \trev~(l_1 \snoc x) $ \\
\hline
$\tmap ~ \cons ~ \snoc ~ \trev$
  & $ \tlen~(\tmap~f~l_1) = \tlen~l_1 $
  & $ \trev~(\trev~l_1) = l_1 $ \\
$\concat ~ \tfold ~ + ~ \tlen$  \\
"stress test"
  & $ \tmap~f~(l_1 \concat l_2) = \tmap~f~l_1 \concat \tmap~f~l_2 $
  & $ \trev~(l_1 \concat l_2) = (\trev~l_2) \concat (\trev~l_1) $ \\
  & $ x \cons \trev~l_1 = \trev~(l_1 \snoc x) $
  & $ \tlen~(l_1 \concat l_2) = \tlen~l_1 + \tlen~l_2 $ \\
  & $ \tfold~f~(\tfold~f~x~l_1)~l_2 = \tfold~f~x~(l_1\concat l_2) $ \\
\hline
\end{tabular}
%
% Up-to-date lemmas from execution logs
\end{comment}
\newcommand\twolines[2]{\renewcommand\arraystretch{1}\begin{array}{@{}l@{}}#1\\#2\end{array}}
\begin{tabular}{@{\hspace{3mm}}l|ll}
$\Vocab$ & \multicolumn{2}{c}{Lemmas discovered} \\
\hline
$0~\tsucc~+$
  & $ x + 0 = x $
  & $ \tsucc~x = x + (\tsucc~0) $ \\
  & $ \tsucc~x + y = x + \tsucc~y $
  & $ (x + y) + z = x + (y + z) $ \\
  & $ x + y = y + x $ \\
\hline
$[]~\cons~\concat~\snoc$
  & $l_1 = l_1 \concat {[]}$
  & $l_1 \concat {(x \cons l_2)} = (l_1 \snoc x) \concat l_2$ \\
  & $l_1 \concat {(l_2\snoc y)} = (l_1 \concat l_2) \snoc y$ 
  & $l_1 \concat {(l_2 \concat l_3)} = (l_1 \concat l_2) \concat l_3$ \\
\hline
$\trev~\cons~\snoc$
  & $x \cons \trev~l_1 = \trev~(l_1 \snoc x)$
  & $\trev~(\trev~l_1) = \trev~l_1$ \\
\hline
$\trev~\snoc~\concat~\cons$
  & $ \trev~(\trev~l_1) = l_1 $
  & $ \trev~(l_1 \snoc x) = x :: \trev~l_1 $ \\
  & $ \trev~(l_1 \concat l_2) = (\trev~l_2) \concat {(\trev~l_1)} $ \\
\hline
$\tfilter$
  & $ \tfilter~p~(\tfilter~p~l_1) = \tfilter~p~l_1 $
  & $ \tfilter~p~(\tfilter~q~l_1) = \tfilter~q~(\tfilter~p~l_1) $ \\
\hline
$\tfilter~\concat$
  & $ \tfilter~p~(\tfilter~p~l_1) = \tfilter~p~l_1 $ 
%  & $ \tfilter~p~(\tfilter~q~l_1) = \tfilter~q~(\tfilter~p~l_1) $   THIS WAS NOT FOUND DUE TO PLACEHOLDER BOUND, RIGHT?
  & $\tfilter~p~(l_1 \concat l_2) = (\tfilter~p~l_1) \concat {(\tfilter~p~l_2)} $ \\
\hline
$0~\tsum~\tfold~+$
  & $\tfold~(+)~0~l_1 = \tsum~l_1$ 
  & $\tfold~(+)~x~l_1 = x + \tsum~l_1$ \\
  & $\tfold~(+)~x~l_1 = x + \tfold~(+)~0~l_1$
  & $x + \tsum~l_1 = x + \tfold~(+)~0~l_1$ \\
\hline
\multirow{2}{*}{$\twolines{\ttrue~\tforall}{\land~\tfold}$}
  & $ \tforall~l_1 = \tfold~(\land)~\ttrue~l_1 $
  & $ \tforall~l_1 \land b = b \land \tfold~(\land)~\ttrue~l_1 $ \\
  & $ \tforall~l_1 \land b = \tfold~(\land)~b~l_1 $
  & $ b \land \tfold~(\land)~\ttrue~l_1 = \tfold~(\land)~b~l_1 $ \\
\hline
\multirow{2}{*}{$\twolines{\tfalse~\texists}{\lor~\tfold}$}
  & $ \tfold~(\lor)~\tfalse~l_1 = \texists~l_1 $
  & $ \tfold~(\lor)~b~l_1 = b \lor \tfold~(\lor)~\tfalse~l_1 $ \\
  & $ \tfold~(\lor)~b~l_1 = \texists~l_1 \lor b $
  & $ b \lor \tfold~(\lor)~\tfalse~l_1 = \texists~l_1 \lor b $ \\
\hline
$\tmap~\circ$
  & $\tmap~g~(\tmap~f~l_1) = \tmap~(g \circ f)~l_1$ \\
\hline
$0~1~+~\trev~\snoc~\tlen$
% Ther ewas a bug in the code. Manual Fix
%   \tlen(\snoc(l_1, 1)) == \tlen(\snoc(l_1, 0))
%   +(1, \tlen(l_1)) == \tlen(\snoc(l_1, y))
%   \tlen(\trev(l_1)) == \tlen(l_1)
%   +(1, \tlen(l_1)) == \tlen(\snoc(l_1, 0))
%   \tlen(\snoc(l_1, x)) == \tlen(\snoc(l_1, 1))
%   \tlen(\snoc(l_1, x)) == \tlen(\snoc(l_1, 0))
%   \tlen(\snoc(l_1, 0)) == \tlen(\snoc(l_1, y))
%   \tlen(\snoc(l_1, 1)) == \tlen(\snoc(l_1, y))
%   +(1, \tlen(l_1)) == \tlen(\snoc(l_1, 1))
%   \tlen(\snoc(l_1, x)) == +(1, \tlen(l_1))
 & $\tlen~l = \tlen~(\trev~l)$
 & $1 + (\tlen~l) = \tlen~(l \snoc x)$ \\
\hline
$+~\concat~\tlen$
  & $ \tlen~(l_1 \concat l_2) = \tlen~l_1 + \tlen~l_2 $ \\
\hline
\multirow{2}{*}{$\twolines{\trev~\tswitch~\ttreeflat}{\ttreemap~\tid}$}
  &  $ t = \ttreemap~\tid~t $
  & $  \tswitch~(\tswitch~t) = t $ \\
  & $  \ttreemap~g~(\tswitch~t) = \tswitch~(\ttreemap~g~t) $ \\
\hline
\multirow{2}{*}{$\twolines{\tmap~\cons~\snoc~\concat}{\tfold~\trev}$}
  & $ \tmap~f~(l_1~\concat~l_2) = (\tmap~f~l_1)~\concat~(\tmap~ f~l_2)$
  & $ \trev~\trev~l = l$ \\
  & $ \tmap~f~(\trev~l) = \trev~(\tmap~f~l)$
  & $ \trev~(l_1 \concat l_2) = (\trev~l_2) \concat (\trev~l_1)$ \\
  & $ \tfold~g~(\tfold~g~x~l_1)~l_2 = \tfold~g~x~(l_1 \concat l_2) $
  & $ x \cons {(\trev~l_1)} = \trev~(l_1\snoc x) $ \\
\hline
\end{tabular} 



==> tables/case-study.tex <==
\newcommand\lright[1]{\multicolumn{1}{r|}{#1}}%
\newcommand\lrighte[1]{\multicolumn{1}{r}{#1}}%
\newcommand\ltime{\lright{\textit{time}}}%
\newcommand\ltimemmss{\lright{\textit{time (mm:ss)}}}%
\newcommand\hhh[1]{{\small#1}}%
\begin{tabular}{l|l|l|l@{}}
$\Vocab$ & \TheSy & Hipster & Leon \\ \hline
\begin{tabular}[t]{@{}p{16mm}@{}}Nat \hfill 1 \\ 0 $\tsucc$ $+$\end{tabular}                                                               & \begin{tabular}[t]{@{}l@{}}x + 0 = x\\ S x = x + (S 0)\\ x + (S y) = S (x + y)\\ (x + z) + y = x + (z + y)\\ z + x = x + z\end{tabular}                                                                              & \begin{tabular}[t]{@{}l@{}}x + 0 = x \\ x + (S y) = S (x + y) \\ (x + z) + y = x + (z + y) \\ z + x = x + z\end{tabular}                                                                                  & \begin{tabular}[t]{@{}l@{}}x + 0 = x \\ x + (S y) = S (x + y) \\ (x + z) + y = x + (z + y) \\ \sout{z + x = x + z}\end{tabular}                                                                                    \\
\ltime                                                                   & \lright{2:04}                                                                                                                                                                                                                 & \lright{2:10}                                                                                                                                                                                                      &      \lrighte{<00:01}                                                                                                                                                                                                       \\
\hline
\begin{tabular}[t]{@{}l@{}}List \hfill 2 \\ rev append\\ cons snoc\end{tabular} & \begin{tabular}[t]{@{}l@{}}xs = xs ++ {[}{]}\\ (xs ++ zs) ++ ys = xs ++ (zs ++ ys)\\ xs :+ y = xs ++ (y::[])\\ rev (rev xs) = xs\\ x::(rev xs) = rev (xs :+ x)\\ rev (xs ++ ys) = (rev ys) ++ (rev xs)\end{tabular} & \begin{tabular}[t]{@{}l@{}}xs = xs ++ {[}{]}\\ x::(rev xs) = rev (xs :+ x)\\ (xs ++ zs) ++ ys = xs ++ (zs ++ ys)\\ rev (xs ++ ys) = (rev ys) ++ (rev xs)\\ rev (z ++ (rev y)) = y ++ (rev z)\end{tabular} & \begin{tabular}[t]{@{}l@{}}xs = xs ++ {[}{]}\\ x::(rev xs) = rev (xs :+ x)\\ (xs ++ zs) ++ ys = xs ++ (zs ++ ys)\\ \sout{rev (xs ++ ys) = (rev ys) ++ (rev xs)}\\ \sout{rev (z ++ (rev y)) = y ++ (rev z)}\end{tabular}   \\
\ltime                                                                   & \lright{16:00}                                                                                                                                                                                                                & \lright{1:36 (18:00)}                                                                                                                                                                                              & \lrighte{<00:01}                                                                                                                                                                                                            \\
\hline
\begin{tabular}[t]{@{}p{16mm}@{}}List \hfill 3a \\ fold sum \\ $+$ $0$\end{tabular}          & \begin{tabular}[t]{@{}l@{}}fold (+) 0 xs = sum xs\\ fold (+) x xs = x + sum xs\\ fold (+) x xs = x + fold (+) 0 xs\\ x + sum(xs) = x + fold (+) 0 xs\end{tabular}                                                    & fold (+) x y = x + (sum y)                                                                                                                                                                                & \begin{tabular}[t]{@{}l@{}}\sout{fold (+) 0 xs = sum xs}\\ \sout{fold (+) x xs = x + sum xs}\\ \sout{fold (+) x xs = x + fold (+) 0 xs}\\ \sout{x + sum(xs) = x + fold (+) 0 xs}\end{tabular}                                           \\
\ltime                                                                   & \lright{10:48 (0:42)}                                                                                                                                                                                                         & \lright{0:34}                                                                                                                                                                                                      &                                                                                                                                                                                                             \\
\hline
\begin{tabular}[t]{@{}p{16mm}@{}}List \hfill 3b \\ map $\concat$ \\ filter\end{tabular}       & \begin{tabular}[t]{@{}l@{}}filter q (filter q xs) = filter q xs\\ \hhh{map f (xs ++ ys) = map f xs ++ map f ys}\\ \hhh{filter p (xs ++ ys) = filter p xs ++ filter p ys}\end{tabular}                                            & \begin{tabular}[t]{@{}l@{}}filt z (filt y x2) = filt y (filt z x2)\\ filt y (filt y z) = filt y z\end{tabular}                                                                                            & \begin{tabular}[t]{@{}l@{}}filt z (filt y x2) = filt y (filt z x2)\\ filt y (filt y z) = filt y z\\ \hhh{map f (xs ++ ys) = map f xs ++ map f ys}\\ \hhh{filter p (xs ++ ys) = filter p xs ++ filter p ys}\end{tabular} \\
\ltime                                                                   & \lright{4:27}                                                                                                                                                                                                                 & \lright{0:13}                                                                                                                                                                                                      &  \lrighte{<00:01}                                                                                                                                                                                                           \\
\hline
\begin{tabular}[t]{@{}p{16mm}@{}}Tree \hfill 4 \\switch \\ tmap id\end{tabular}            & \begin{tabular}[t]{@{}l@{}}t = tmap id t\\ switch (switch t) = t\\ tmap f (switch t) = switch (tmap f t)\end{tabular}                                                                                                & \begin{tabular}[t]{@{}l@{}}switch (switch y) = y\\ tmap id y = y\\ tmap y (switch z) = switch (tmap y z)\end{tabular}                                                                               & \begin{tabular}[t]{@{}l@{}}switch (switch y) = y\\ tmap id y = y\\ tmap y (switch z) = switch (tmap y z)\end{tabular}                                                                                 \\
\ltime                                                                   & \lright{0:15}                                                                                                                                                                                                                 & \lright{0:24}                                                                                                                                                                                                      &  \lrighte{<00:01}                                                                                                                                                                                                           \\
\hline
\begin{tabular}[t]{@{}l@{}}Conditions \\leq \hfill 5\end{tabular}                                                                    & n/a                                                                                                                                                                                                                  & \begin{tabular}[t]{@{}l@{}}leq x x\\ leq x (Succ x)\\ not (leq (Succ x) x)\\ leq y x $\Rightarrow$ not (leq (Succ x) y)\\ leq x y $\Rightarrow$ leq x (Succ y)\end{tabular}                               & \begin{tabular}[t]{@{}l@{}}\sout{leq x x}\\ \sout{leq x (Succ x)}\\ \sout{not (leq (Succ x) x)}\\ \sout{leq y x $\Rightarrow$ not (leq (Succ x) y)}\\ \sout{leq x y $\Rightarrow$ leq x (Succ y)}\end{tabular}                                 \\
\ltime                                                                   &                                                                                                                                                                                                                     & \lright{12:39}                                                                                                                                                                                                     &                                                                                                                                                                                                            
\\
\hline
\end{tabular}

==> tables/experiment-stats.tex <==
\begin{tabular}{|l|r|r|rr|rrr|}
\hline
          & \multicolumn{4}{c|}{Time (\textit{sec})}                           & \multicolumn{3}{c|}{Lemmas} \\
          &  Generation  &             & \multicolumn{2}{c|}{Induction Prover} & & &        \\
$\Vocab$  &  + Inference &   Filtering & \hspace{1cm}  & {\small(retries)}     & found\!\! & failed\!\! & retried\!\!    \\ \hline
$0~\tsucc~+$                                  &         30.89  &        92.74     &            3     &         0.00     &      5 &     0 &      0  \\
\hline
$[]~\cons~\concat~\snoc$                      &       2692.57  &       293.33     &           <1     &         0.00     &      4 &     0 &      0  \\
\hline
$\trev~\cons~\snoc$                           &         13.01  &         2.27     &           <1     &         0.09     &      2 &     1 &      1  \\
\hline
$\trev~\snoc~\concat~\cons$                   &       1444.45  &        10.68     &           <1     &         0.10     &      3 &     1 &      1  \\
\hline
$\tfilter$                                    &          1.34  &         1.12     &           <1     &         0.00     &      2 &     0 &      0  \\
\hline
$\tfilter~\concat$                            &         30.20  &         5.04     &            1     &         0.00     &      2 &     8 &      0  \\
\hline
$0~\tsum~\tfold~+$                            &        445.00  &       188.28     &            1     &         0.30     &      4 &     2 &      1  \\
                                              &         (26.32)  &        (12.80)     &            (3)     &         (0.33)     &        &     (2) &      (1)  \\
\hline
$\ttrue~\tforall~\land~\tfold$                &        501.94  &       169.13     &            3     &         1.07     &      4 &     3 &      2  \\
                                              &         (15.02)  &        (12.31)     &            (1)     &         (0.92)     &        &     (3) &      (2)  \\
\hline
$\tfalse~\texists~\lor~\tfold$                &        517.29  &       231.81     &            2     &         0.34     &      4 &     2 &      1  \\
                                              &         (30.57)  &        (27.26)     &            (3)     &         (1.19)     &        &     (3) &      (2)  \\
\hline
$\tmap~\circ$                                 &          3.66  &         0.87     &           <1     &         0.00     &      1 &     0 &      0  \\
\hline
$0~1~+~\trev~:+~\tlen$                        &        162.44  &        34.61     &           48     &        41.64     &     10 &     2 &      1  \\
\hline
$+~\concat~\tlen$                             &         39.66  &         5.15     &           <1     &         0.00     &      1 &     0 &      0  \\
\hline
 $\trev~\tswitch~\ttreeflat~\ttreemap~\tid$    &          7.76  &         1.54     &            1     &         0.00     &      3 &     0 &      0  \\
\hline
$\tmap~\cons~\snoc~\concat~\tfold~\trev$      &      15020.65  &        33.70     &            2     &         0.94     &      7 &     3 &      3  \\
\hline
\end{tabular}

==> tables/time_percentiles.tex <==
\renewcommand\arraystretch{1.3}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l@{~~~}|r|r|r|r|r|r|r|r|r|r|}
\cline{2-11}
\multicolumn{1}{l|}{}
                              & 10\%         & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 100\% \\ \hline
\TheSy   & \textless{}1 & 2    & 6    & 12   & 46   & 113  & 792  & 8.3K & 39K  & 68K   \\ \hline
Hipster  & 380          & 1.3K & 3K   & 5.2K & 7.8K & 11K  & 16K  & 23K  & 34K  & 47K   \\ \hline
\end{tabular}
\vspace{3pt}

==> todo.tex <==
Abstract
    Explain why the title says "Deductive Synthesis" - V
Intro - 
    change order - V
    add abstraction text - V
    fix example to something TheSy manages and quick* doesn't - V
    Contributions should include: We created thesy which overcomes all noted limitations - V
    Contribution is not the metric but rather the evaluation - V
    Remove the 100x and orders of magnitude - V
Overview -
    Fixup the two overview lists - ignored
    Add fourth loopback to second list - V
    Add short comment on case split shortcomings - V
Related work - 
    Smt backtracking
    "Combining the Top-down Propagation and Bottom-up Enumeration for Inductive Program Synthesis" POPL2021
Results - 
    Fix case split text - V 
    Run the *@#!ing experiments - V
    Change explanation for the speed graph
Future/Limitations - 
    Do case splitting right
    
Link to repo
    
Many many many revisions on the text to fix it up.
